Cache-Aided Asymmetric MIMO Communications: Achievable DoF Analysis

Integrating coded caching (CC) into multiple-input multiple-output (MIMO) communications significantly enhances the achievable degrees of freedom (DoF). This paper investigates a practical cache-aided asymmetric MIMO configuration with cache ratio $\gamma$, where a server with $L$ transmit antennas communicates with $K$ users. The users are partitioned into $J$ groups, and each user in group $j$ has $G_j$ receive antennas. We propose four content-aware MIMO-CC strategies: \emph{min-$G$} enforces symmetry using the smallest antenna count among users; \emph{Grouping} maximizes intra-subset spatial multiplexing gain at the expense of some global caching gain; \emph{Super-grouping} aggregates users into optimized \emph{min-$G$}-based super-sets with identical effective receive multiplexing gains before applying \emph{Grouping} across them; and \emph{Phantom} redistributes spatial resources assuming "phantom" antennas at the users to bridge the performance gains of \emph{min-$G$} and \emph{Grouping}. We develop these asymmetric strategies under three reference symmetric CC placement-delivery policies with guaranteed linear decodability: a finite-search DoF-optimized policy attaining the best single-shot achievable DoF lower bound, and two closed-form policies, namely combinatorial and linear cyclic low-complexity constructions, with the cyclic policy attaining DoF performance close to the others in many operating regimes. Analytical and numerical results demonstrate significant DoF improvements across various system configurations, and that policy-strategy combinations offer flexible trade-offs between DoF and subpacketization complexity.

==> Figs/DoF_Prop_SOTA.tex <==
L		minGopt		minGsbopt		groupingop		groupingopeff		groupingsbop		groupingsbopeff			phantomopt		phantomsbopt	
																		
10		28		28		2.55E+01		3.39E+01		2.16E+01		3.18E+01			38.08		36	
11		30		28		27.7169		3.55E+01		21.6		3.18E+01			40.41		38.08	
12		30		30		28.7452		3.55E+01		26.5108		3.53E+01			41.54		39.08	
13		32		30		30.8571		3.95E+01		26.5108		3.53E+01			44.57		42.2	
14		32		32		32.459		3.95E+01		27.2269		3.74E+01			45.82		43.31	
15		34		32		33.9267		4.15E+01		27.2269		3.74E+01			46.96		44.33	
16		34		34		34.9461		4.15E+01		31.0048		3.92E+01			48		45.63	
17		36		34		36.8301		4.42E+01		31.0048		4.05E+01			49.46		47.24	
18		36		36		37.9391		4.42E+01		33.2308		4.34E+01			50.82		48.49	
19		38		36		38.6803		4.75E+01		33.2308		4.34E+01			53.57		49.66	
20		38		38		39.8212		4.75E+01		34.8899		4.50E+01			54.42		51.43	


==> Figs/DoF_Prop_T1_1.tex <==
K2		minG		grouping		supgrouping			phantom		MUMIMO		supgroupingcpar			groupingcpar			phantomcpar			minGcpar		groupinglpar		phantomlpar	
																											
																											
5		28		25.6941		25.6941			28		12		23.8689			23.8689			28			28		23.8689		28	
10		28		25.8462		25.8462			28		12		24			24			28			28		25.0213		28	
15		28		27.2566		27.2566			28		12		25.4021			25.4021			28			28		22.8148		28	
20		28		30		30			28		12		28			28			28			28		22.1053		28	
25		28		34.9307		34.9307			34.25		12		32.5161			32.5161			 32.8404			28		21.9130		28	
30		28		36.1290		36.1290			46.42		12		33.7931			33.7931			43.1748			28		 21.1628		28	


==> Figs/DoF_Prop_T1_2.tex <==
K2		minG		grouping		supgrouping			phantom		MUMIMO		supgroupingcpar			groupingcpar			phantomcpar			minGcpar		groupinglpar		phantomlpar	
																											
																											
5		28		25.6941		25.6941			28		    12		23.8689			23.8689			18.9890			28		23.8689		28	
10		28		25.8462		25.8462			28		    12		24			      24			19.1390			28		25.0213		28	
15		28		27.2566		27.2566			28		    12		25.4021			25.4021			21.7173			28		22.8148		28	
20		28		30		      30			28		    12		    28			28			     25.9239		    28		22.1053		28	
25		28		34.9307		34.9307			34.25		12		32.5161			32.5161			 32.3299	28		21.9130		28	
30		28		36.1290		36.1290			40.6452		12		33.7931			33.7931		     37.9661	28		21.1628		28	


==> Figs/DoF_Prop_T2.tex <==
K2		minG		grouping		supgrouping			phantom			Upbsym		MUMIMO		supgroupingcpar			groupingcpar			Upbsymcpar
																						
																						
0		36		NaN		36			36			36		24		36			NaN			36
10		36		34.1627		36			36			42		24		36			 33.6495			42
20		36		34.7586		36			36			48		24		36			34.2857			48
30		36		37.2152		37.2152			36			55		24		36.9231			36.9231			50
40		36		42		42			41.14			60		24		42			42			60
50		36		46.8293		46.8293			52.36			70		24		46.8293			46.8293			63
60		72		NaN		72			72			72		24		72			NaN			72


==> Figs/DoF_Prop_gamma5.tex <==
gamma		minGopt		groupingop		groupingopeff		phantomopt
								
0.02		 30.80		31.4758		43.7790		47.652
0.04		45.60		42.8142		62.9731		66.6860
0.06		60.40		52.4875		79.1422 		81.6660
0.08		75.20		61.2280		93.7151		93.0760
0.1		90		69.6801		107.3433		102.07
0.2		164		110.8793		169.3435		164


==> Figs/DoF_Prop_gamma6.tex <==
gamma		minGopt		groupingop		groupingopeff		phantomopt
								
0.02		 30.80		30.6986		38.6996		42.7300
0.04		45.60		40.8449		54.3847		57.4820
0.06		60.40		49.6903		68.1924		72.6420
0.08		75.20		57.6772 		81.2279		85.7340
0.1		90		65.4033		93.8712 		96.89
0.2		164		103.0987 		154.9159		164


==> Figs/DoF_Scalability3.tex <==
Scen		minGopt		groupingopeff		phantomopt
						
sp1		34		34		34
sp2		34		34.7368		38.2
sp3		34		39.1111		40.32
sp4		34		40.5		44.78
sp5		36		45.2055		52.56
sp6		56		57.931		68.68
sp7		36		72.7941		75.79


==> Figs/DoF_effgrp_phantom_senseitivity.tex <==
Scen    minGsbopt   groupingsbop   groupingsbopeff   phantomsbopt   phantomsimpbopt
sp1a    42.0000     42.0000        42.0000           43.5556        43.5561
sp1b    42.0000     42.0000        42.0000           43.5556        45.2177

sp2a    24.0000     24.9500        25.4550           26.6667        27.0233
sp2b    24.0000     23.8020        24.6150           25.6000        26.4551

sp3a    27.0000     22.5980        28.8600           30.5455        30.8297
sp3b    24.0000     18.5130        24.7500           26.6667        27.0632

sp4a    36.0000     37.6660        39.4483           41.1429        41.9634
sp4b    36.0000     35.3541        39.4483           41.1429        41.6664

==> Figs/DoF_imp_over_prim1.tex <==
Scen		minGsbopt		groupingsbop		groupingsbopeff		phantomsbopt		phantomsimpbopt
										
sp1		35		32.8276		35		36.7761		37.35
sp2		45		40.4278		49.7368		50.5263		50.5263
sp3		52		 49.1707		60.9677		68.87		68.87
sp4		52		52.2198		65.3945		67.20		67.20
sp5		88		78.9254		98.4142 		89.14		89.14

